ViHOS: Hate Speech Spans Detection for Vietnamese

The rise in hateful and offensive language directed at other users is one of the adverse side effects of the increased use of social networking platforms. This could make it difficult for human moderators to review tagged comments filtered by classification systems. To help address this issue, we present the ViHOS (Vietnamese Hate and Offensive Spans) dataset, the first human-annotated corpus containing 26k spans on 11k comments. We also provide definitions of hateful and offensive spans in Vietnamese comments as well as detailed annotation guidelines. Besides, we conduct experiments with various state-of-the-art models. Specifically, XLM-R$_{Large}$ achieved the best F1-scores in Single span detection and All spans detection, while PhoBERT$_{Large}$ obtained the highest in Multiple spans detection. Finally, our error analysis demonstrates the difficulties in detecting specific types of spans in our data for future research. Disclaimer: This paper contains real comments that could be considered profane, offensive, or abusive.

==> sections/backup.tex <==
\section{Abusive Language Characteristics}
\label{appendix_A}

%\onecolumn
% \setlength\LTleft{0pt}            % default: \fill
% \setlength\LTright{-1pt}           % default: \fill
\begin{center}
\begin{longtable}{|l|l|l|}
%{|l|l|l|} p{0.2\linewidth}|p{0.4\linewidth}|p{0.4\linewidth}
\hline \multicolumn{1}{|l|}{\textbf{Characteristics}} &
\multicolumn{1}{l|}{\textbf{Examples}} &
\multicolumn{1}{l|}{\textbf{Explanation and Solutions}} \\ \hline 
\endfirsthead 

\multicolumn{3}{l}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline \multicolumn{1}{|l|}{\textbf{Characteristics}} &
\multicolumn{1}{l|}{\textbf{Examples}} &
\multicolumn{1}{l|}{\textbf{Explanation and Solutions}} \\ \hline 
\endhead

\hline \multicolumn{3}{|r|}{{Continued on next page}} \\ \hline
\endfoot

\hline
\endlastfoot

\pbox{0.38\linewidth}{Non-diacritical marks comments}                 & \pbox{0.75\linewidth}{(1) Dit me cai quy trinh,vao cap cuu deo co tien,deo bao hiem thi nam do di. \\ (\textbf{Eng:} \textit{Fuck the procedure, without money or insurance, you could just lay there and no one cares about your emergency}\\ (2) Dung la con linh dien dien vua thoi chang qua nt goi de choc my dien thoi "con ng" nhu linh dien thi ai them\\ (\textbf{Eng:} \textit{That must be the Crazy Linh, so crazy! I just call to tease the Crazy My. No one gonna love Crazy/The person like Crazy Linh!}}               & \pbox{0.75\linewidth}{\textbf{Explanation:} some of these non-diacritical marks comments might trick annotators a little bit. \\ (1): this is a non-diacritic comment but still able to understand. \\ (2): there are some problems causing annotators to re-read multiple times as no punctuation, diacritic, and the text "con ng" could be considered as "crazy girl" or "the type (of human)" and both of these meanings is inappropriate.\\ \\ \textbf{Solution:} non-diacritic comments are annotated as others. Annotators have to re-read until they fully understand the texts if needed. Those examples are annotated as follows:\\ (1): {[}"Dit me",  "deo", "deo"{]}\\ (\textbf{Eng:}  {[}"\textit{Fuck}",  "\textit{fuck}", "\textit{fuck}"{]})\\ (2): {[}"con", "dien", "dien", "con ng",  "dien", "ai them"{]}\\ (\textbf{Eng:}  {[}"\textit{con}",  "\textit{crazy}", "\textit{crazy}", "\textit{crazy/the person like}",  "\textit{crazy}", "\textit{No one gonna love}"{]} in which the word "con" is an inappropriate way to call a woman.)} \\ \hline
\pbox{0.38\linewidth}{Metaphors, metonymy}                          & \pbox{0.75\linewidth}{(1) cái miệng rộng quá đẻ con ra còn lọt\\ (\textbf{Eng:} \textit{The mouth is too big that a baby could even be born through it})\\ (2) Dm! qua đợt dịch này thì thằng sống ích kỷ này chắc sớm gia nhập juventuts\\ (\textbf{Eng:} \textit{Fuck it! After the pandemic, this selfish boy will soon join Juventuts})}                                                     & \pbox{0.75\linewidth}{\textbf{Explanation:} in our dataset, many comments use metaphors or metonymy to convey their hate or offensiveness in another way. \\ (1): this is a metaphor of a mouth as a vagina.\\ (2): this is a metonymy of Juventus jersey as prison shirts (a common metonymy in Vietnamese).\\ \\ \textbf{Solution:} Annotators are required to annotate the whole ideas of metaphors, metonymy.\\ (1):  {[}"cái miệng rộng quá đẻ con ra còn lọt"{]}\\ (2):  {[}"Dm", "thằng sống ích kỷ này chắc sớm gia nhập juventuts"{]}\\ (\textbf{Eng:}  {[}"\textit{Fuck}",  "\textit{this selfish boy will soon join Juventuts}"{]})}                                            \\ \hline
\pbox{0.38\linewidth}{Puns}                                           & \pbox{0.75\linewidth}{(1) Ad đăng bài này cũng là Bồn Kỳ Lắc nè nè nè :) \\ (\textbf{Eng:} \textit{The admin, who posts this, is also a "Bồn Kỳ Lắc{\ttfamily" :)}})} & \pbox{0.75\linewidth}{\textbf{Explanation:} Some comments use phrases that only read them backwards, they make sense. As in the example, "Bồn Kỳ Lắc", if this phrase is read backwards, it is "Bắc Kỳ Lồn" (pussy north).\\ \\ \textbf{Solution:} Annotators are required to annotate these puns too.\\ (1):  {[}"Bồn Kỳ Lắc"{]}}\\ \hline
\pbox{0.38\linewidth}{Using non-words characters to form hieroglyphs} & \pbox{0.75\linewidth}{(1) có tin t lấy {\fontspec{Symbola}\symbol{"1F52A}} xiên chết cụ m ko :)))\\ (\textbf{Eng:} \textit{Do you belive that I could get a {\fontspec{Symbola}\symbol{"1F52A}} to fucking kill you?})\\ (2) Đâm vào () \\ (\textbf{Eng:} \textit{stab in the ()})}  & \pbox{0.75\linewidth}{\textbf{Explanation:} \\ (1): the icon {\fontspec{Symbola}\symbol{"1F52A}} is used instead of the word knife. \\ (2): the existence of "()" can be considered as pussy in this context.\\ \\ \textbf{Solution:} Annotating the non-words only if they can convey a full meaning of hate or offensiveness, and the whole phase if they can not.\\ (1): {[}"t", "{\fontspec{Symbola}\symbol{"1F52A}}", "xiên chết cụ m""{]}\\ (\textbf{Eng:}  {[}"\textit{t}",  "\textit{{\fontspec{Symbola}\symbol{"1F52A}}}", "\textit{fucking kill you}"{]}) in which "t", "m" are inappropriate pronouns.)\\ (2): {[}"Đâm vào ()""{]}}                                                                                                                \\ \hline
\pbox{0.38\linewidth}{Spelling mistakes}                              & \pbox{0.75\linewidth}{(1) Tôi đeo hiểu bạn noi cai gì luôn a :))) \\ (\textbf{Eng:} \textit{I have no fucking idea about what you saying})\\ (2) Mà dx cái chữi ngta nghe hài vcl bù lại củng đở  \\ (\textbf{Eng:} \textit{Those fucking curses is so funny that can even refill that})\\
(3)Khi bạn xai trính tã nhưng cá ghén vít đún trính tã :))\\ (\textbf{Eng:} \textit{When you make spelling mistakes but trying to fix it :))})}                                                  & \pbox{0.75\linewidth}{\textbf{Explanation:} \\ (1): the words "đeo," "noi," "cai," "a" are spelling mistakes. The words can be understood as "đéo," "nói," "á". As that, these words are the same in accidentally missing acute marks. \\ (2): the words: "chữi," "củng," "đở" are spelling mistakes is a phenomenon of mistaking tilde mark for hook above mark, and this often happens in some parts of Vietnam \cite{nguyenhoainguyen}. There are also familiar phenomena of mistaking marks such as tilde mark for underdot mark, acute mark for hook above mark, and so on \cite{nguyenhoainguyen}. \\ (3): the phases: "xai trính tã," "cá ghén," "vít đúng trính tã" are spelling mistakes but on purpose. This comment utilizes spelling mistakes to attack opponents who also have spelling mistakes. Furthermore, these spelling mistakes also abuse opponents based on regional distinctions in accent, which cause some phenomenon of mistaking diacritical marks as in Example (2).\\ \\ \textbf{Solution:} As with non-diacritical marks, annotators work as usual.\\ (1): {[}"deo"{]}\\ (\textbf{Eng:}  {[}"\textit{fuck}"{]})\\ (2): {[}"chữi", "vcl"{]}\\ (\textbf{Eng:}  {[}"\textit{curse}", "\textit{fuck}"{]})\\ (3): {[}"bạn xai trính tã nhưng cá ghén vít đún trính tã :))"{]}} \\ \hline
\pbox{0.38\linewidth}{Profound}                                       & \pbox{0.75\linewidth}{ra gì thì toi rồi, nó khác gì cách đảng CS chọn người, hồng hơn chuyên. Suy nghĩ kĩ đi. Giải độc cộng sản đã khó, giải độc tư tưởng cánh tả còn khó hơn.\\ (\textbf{Eng:} \textit{If it had something, it was done! It is just like the way CS (stands for Communism) chooses people, beauty over the profession. Detoxifying Communism is hard; detoxifying the left-wing political ideologies is even harder.})} & \pbox{0.75\linewidth}{\textbf{Solution:} Annotators are required to annotate the whole profound abuse.\\ (1): {[}"toi", "hồng hơn chuyên", "Giải độc cộng sản đã khó, giải độc tư tưởng cánh tả còn khó hơn"{]}\\ (\textbf{Eng:}  {[}"\textit{die}", "\textit{beauty over the profession}", "\textit{Detoxifying Communism is hard; detoxify the left-wing political ideologies even harder}"{]})\\ (2): {[}"Rút kinh nghiệm lại được xài nghìn tỷ"{]}}                                    \\ \hline
\pbox{0.38\linewidth}{Homonym}                                        & \pbox{0.75\linewidth}{(1) coin card \\ ("coin card" is homonym to "con cặc" which means \textit{dick})} & \pbox{0.75\linewidth}{\textbf{Solution:} annotate the whole homonym abuse.\\ (1): {[}"coin card"{]}}    \\ \hline
\pbox{0.38\linewidth}{Mixing languages}                               & \pbox{0.75\linewidth}{Vl fake\\ (\textbf{Eng:} Fuck! Fake)\\ phe Nguyễn Phú Trọng compat tổng Nguyễn Tấn Dũng =))\\ (\textbf{Eng:} \textit{Nguyen Phu Trong side combat Nguyen Tan Dung side})\\ Tối Thầy stream đá phò đi thầy ơi\\ (\textbf{Eng:} \textit{You should stream fucking some whores tonight, please!})} & \pbox{0.75\linewidth}{\textbf{Solution:} treat foreign words as others and annotate if they meet the definition of hate and offensiveness.\\ (1): {[}"Vl", "fake"{]}\\ (\textbf{Eng:}  {[}"\textit{fuck}", "\textit{fake}"{]})\\ (2): {[}"compat"{]}\\ (\textbf{Eng:}  {[}"\textit{combat}"{]})\\ (3): {[}"đá phò"{]}\\ (\textbf{Eng:}  {[}"\textit{fuck some whores}"{]})}     \\ \hline
\pbox{0.38\linewidth}{Trick hate speech detecting systems on purpose} & \pbox{0.75\linewidth}{Đấy Ông già xạo l*n của các bạn được tắm bồn Thái Lan đấy=)))\\ (\textbf{Eng:} \textit{See, your fucking old liar is Thai bathing again =)))})\\ thằng  c h.ó ngu\\ (\textbf{Eng:} \textit{Fucking stupid guy})\\ vualonemlabaonhieu cm\\ (\textbf{Eng:} \textit{How long in cm to fit your pussy?})} & \pbox{0.75\linewidth}{\textbf{Explanation}: some hate or offensive comments use punctuation to censor their inappropriate words (as in (1), asterisk is used in the word l*n (pussy)) or to disunite characters in words (as in (2), dot and space are used to disunite the words chó (dog) into c h.ó). \\ These efforts actually can trick many hate speech detecting systems, or to put all together (as in (3),  vualonemlabaonhieu cm should be "vừa lồn em là bao nhiêu cm").\\ \\ \textbf{Solution:} we annotate all characters which can be form into hate or offensive phase.\\ (1): {[}"xạo l*n"{]}\\ (\textbf{Eng:}  {[}"\textit{fucking lie}"{]})\\ (3): {[}"thằng  c h.ó", "ngu"{]}\\ (1): {[}"lon"{]}\\ (\textbf{Eng:}  {[}"\textit{pussy}"{]})}\\ \hline
%\bottomrule \addlinespace
\caption[Characteristic of abusive language in ViHOS with Examples, Explanation, and Solution for annotators.]{Characteristic of abusive language in ViHOS with Examples, Explanation, and Solution for annotators.}
\label{tab:cmt_Characteristic}
\end{longtable}
\end{center}


\section{Addition notices for annotators}

\begin{longtable}{|l|l|l|}
\hline \multicolumn{1}{|l|}{\pbox{0.6\linewidth}{\textbf{Notices}}} &
\multicolumn{1}{l|}{\pbox{0.6\linewidth}{\textbf{Examples}}} &
\multicolumn{1}{l|}{\pbox{0.6\linewidth}{\textbf{Explanation}}} \\ \hline 
\endfirsthead

\multicolumn{3}{l}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline \multicolumn{1}{|l|}{\pbox{0.6\linewidth}{\textbf{Notices}}} &
\multicolumn{1}{l|}{\pbox{0.6\linewidth}{\textbf{Examples}}} &
\multicolumn{1}{l|}{\pbox{0.6\linewidth}{\textbf{Explanation}}} \\ \hline 
\endhead

\hline \multicolumn{3}{|r|}{{Continued on next page}} \\ \hline
\endfoot

\hline
\endlastfoot

\pbox{0.65\linewidth}{Try to figure out and consider as in the original context of the comments.}   &  & \pbox{0.60\linewidth}{This could help annotators understand complex and non-context hate, offensive comments.}\\ \hline
\pbox{0.65\linewidth}{Do not let emotion affect the annotating process.} &  & \pbox{0.60\linewidth}{Annotators exposed in a long time to toxic comments are reported to get used to the frequently appearing hate, offensiveness.}    \\ \hline
\pbox{0.65\linewidth}{Check the provided Vietnamese Dictionary if there is any uncertainty in being sure a word is hate or offensive or a rare word.}                       &   & \pbox{0.60\linewidth}{We use the most reputable Vietnamese dictionary \cite{hoangphe} to provide to annotators}\\ \hline
\pbox{0.65\linewidth}{Should span the object is compared to in an inappropriate comparison.}         & \pbox{0.60\linewidth}{"Ăn cơm nhìn như chó"\\ (\textbf{Eng:} \textit{You eat like a dog}) \\ \textbf{Spans:} {[}"Ăn cơm nhìn như chó"{]}} & \pbox{0.60\linewidth}{We consider this is an inappropriate comparison in which annotators must span "chó"$_{dog}$.} \\ \hline
\pbox{0.65\linewidth}{However, we should span the whole comparison if spanning only the object is compared to might not convey the complete hate or offensive idea}         & \pbox{0.60\linewidth}{"ý thức như trẻ lớp mầm"\\ (\textbf{Eng:} \textit{Your awareness is just like a kindergarten kid}) \\ \textbf{Spans:} {[}"ý thức như trẻ lớp mầm"{]}} & \pbox{0.60\linewidth}{If we only span "trẻ lớp mầm"$_{\text{kindergarten kid}}$, it will not convey the complete offensive idea. As that, annotators are encouraged to span the whole text instead.}  \\ \hline
\pbox{0.65\linewidth}{Do not span conjunctions; exceptional Vietnamese cases; the standard way to call LGBTQ+.} & \pbox{0.60\linewidth}{(1) Vì thế, nên, nhưng, mà, etc.\\ (\textbf{Eng:} \textit{so, so, but, but, etc.}) \\  (2) Gay, les, etc\\ (3) Bóng, bê đê, ái nam ái nữ, etc.}          & \pbox{0.60\linewidth}{(1) Some conjunctions in Vietnamese.\\ (2) Appropriate ways to specify LGBTQ+.\\ (3) Inappropriate ways to specify LGBTQ+ that need to be spanned in comments.}\\ \hline
\pbox{0.65\linewidth}{Blatant hate and offensive words prioritize being spanned over the others, especially in sentences without diacritics and could not be understanded.} & \pbox{0.60\linewidth}{May Cha H O an Tro. Cap. Ranh c. Di ngoi le. Nhieu chuyen. Do  Cai Thu ,  do tam than\\ \textbf{Spans:} {[}"Cap", "ngoi le", "Nhieu chuyen", "do tam than"{]}\\ (\textbf{Eng:} {[}"\textit{steal}", "\textit{gossip}", "\textit{talkative}", "\textit{psycho}"{]})} & \pbox{0.60\linewidth}{Similar to this non-diacritical marks and inapprehensible comment, annotated spans are more straightforward to be spanned.}\\ \hline
\pbox{0.65\linewidth}{Span the whole phase violating human rights.} & \pbox{0.60\linewidth}{"Về nước anh nên vào tù ở trước thay vì đi cách ly." \\ (\textbf{Eng:} \textit{When you return to Vietnam, you should go to jail first instead of going to isolation}) \\ \textbf{Spans:} {[}"Về nước anh nên vào tù ở trước thay vì đi cách ly"{]}} & \pbox{0.60\linewidth}{Comments violate human rights, usually complex to specify hate, offensive words to span. As in this example, a Vietnamese citizen comes back from a foreign country has a right to have isolated healthcare firstly.} \\ \hline
\pbox{0.65\linewidth}{Span the whole obscene acronyms.} & \pbox{0.60\linewidth}{(1) clgv \\ (\textbf{Eng:} \textit{wtf is that?}) \\ (2) clmn \\ (\textbf{Eng:} \textit{your mom’s pussy}) \\ (3) cmn \\ (\textbf{Eng:} \textit{your mother}).} &   \\ \hline
\pbox{0.65\linewidth}{Follow the rule with words that do not have diacritics and conjoin to span out the hate, offensive spans.} & \pbox{0.60\linewidth}{cailongithe \\ (\textbf{Eng:} \textit{wtf is that?}) }& \pbox{0.60\linewidth}{Some comments have string being constructed by many non-diacritic words,  but still able to understand. The annotators should only span the hate and offensive set out of the string as in the example.}    \\ \hline
\pbox{0.65\linewidth}{Span separately.}  & \pbox{0.60\linewidth}{"Cả đám dlv là nhóm ngu dốt, trẻ trâu potay vcl luôn." \\ (\textbf{Eng:} \textit{The whole dlv crew are stupid, bull-headed kids (so I have) no fucking thing to say.})\\ \textbf{Spans:} {[}"đám", "ngu dốt", "trẻ trâu"{]}\\ (\textbf{Eng:} {[}"\textit{crew}", "\textit{stupid}", "\textit{bull-headed kids}"{]})} & \pbox{0.60\linewidth}{This comment must be spanned as in the example, but not as "đám", "ngu dốt, trẻ trâu".}\\ \hline
\caption[Additional notices for annotators.]{Additional notices for annotators.} \label{tab:ann_notices}
\end{longtable}

\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/err12.png} 
    \caption{Several types of error and corresponding examples.}
    \label{fig:error}
\end{figure*}

\begin{table*}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{m{0.35\textwidth}||m{0.15\textwidth}|m{0.15\textwidth}||m{0.15\textwidth}}
\hline
\multirow{2}{*}{\textbf{Content }}                                                                                                                                                                                                                                                                                                                         & \multicolumn{2}{c||}{\textbf{Models }}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Gold spans}}}                                                                                                                                                                                                                                                                                                                           \\ 
\cline{2-3}
                                                                                                                                                                                                                                                                                                                                                           & \multicolumn{1}{c|}{PhoBERT$_{Large}$}                                                                                                                                                                                                                                                                  & \multicolumn{1}{c||}{XLM-R$_{Large}$}                                                                                                                                                                                                                                                      & \multicolumn{1}{c}{}                                                                                                                                                                                                                                                                                                                                                               \\ 
\hline
\pbox{0.35\textwidth}{Ns vậy lại xúc phạm cái \hl{đầu b**i} *neutral face emoji*\\(\textbf{Eng}: \textit{If you said so, you insult the \hl{d**k head}~*neutral face emoji*})}                                                                                                                                                                      & \pbox{0.15\textwidth}{{[}"xúc", "đầu"]\\(\textbf{\textbf{Eng}}: [\textit{no meaning when standing alone}, "\textit{head}"])}                                                                                                                                                                & \pbox{0.15\textwidth}{{[}"b**i"]\\(\textbf{\textbf{\textbf{\textbf{Eng}}}}: ["\textit{d**k}"])}                                                                                                                                                                                & \pbox{0.15\textwidth}{{[}"đầu b**i"]\\(\textbf{\textbf{\textbf{\textbf{Eng}}}}: ["\textit{d**k~head}"])}                                                                                                                                                                                                                                                          \\ 
\hdashline
\pbox{0.35\textwidth}{@username nhân dân VN tức là cờ đỏ. Còn đám cờ vàng là lũ súc vật lưu vong. Hiểu hông?\\(\textbf{\textbf{Eng}}: \textit{@username Vietnamese people are red flag. The yellow flag ones are animals and exiled. Understand?})}                                                                                       & \pbox{0.15\textwidth}{{[}"đỏ.", "đám", "lũ", "súc"]\\(\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{Eng}}}}}}}}: ["\textit{red}", "\textit{those}", "\textit{those}",~\textit{no meaning when standing alone}])}                                                          & \pbox{0.15\textwidth}{{[}"đám", "lũ", "súc", "vật", "vong."]\\(\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{Eng}}}}}}}}}}}}}}}}: ["those", "\textit{those}",~\textit{"animals", "died."}])} & \pbox{0.15\textwidth}{{[}"đám cờ vàng", "lũ súc vật lưu vong."]\\(\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{Eng}}}}}}}}}}}}}}}}: ["\textit{the yellow flag ones}", "\textit{animals and exiled"}])}                                                                         \\ 
\hdashline
\pbox{0.35\textwidth}{Cướp đêm là giặc, cướp ngày là quan. 24/7 lúc nào cũng phải nơm nớp. Than ôi cái đất nước hạnh phúc\\(\textbf{\textbf{\textbf{\textbf{Eng}}}}:~\textit{Night thieves~are enemies, day thieves are bureaucrats. 24/7, we are in a~ perpetual state of fear and anxiety. What a happy country})}                      & \pbox{0.15\textwidth}{{[}"Cướp", "cướp", "nớp."]\\(\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{Eng}}}}}}}}}}}}}}}}: ["\textit{thieves}", "\textit{thieves}",~\textit{no meaning when standing alone}])} & \pbox{0.15\textwidth}{{[}"Cướp", "giặc,", "cướp"]\\(\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{Eng}}}}}}}}}}}}}}}}: ["\textit{thieves}", "\textit{enemies}", "\textit{thieves}"])}        & \pbox{0.15\textwidth}{{[}"Cướp đêm là giặc, cướp ngày là quan.", "Than ôi cái đất nước hạnh phúc"]\\(\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{Eng}}}}}}}}}}}}}}}}: ["\textit{Night thieves~are enemies, day thieves are bureaucrats}", "\textit{What a happy country}"])}  \\ 
\hdashline
\pbox{0.35\textwidth}{Đúng rồi đéo thể tin được. Đáng lẽ phải cào bằng ra mới đúng. Thật không thể tin nổi. Phải cào bằng ra mới được\\(\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{Eng}}}}}}}}: \textit{Yes, fucking unbelievable. They should dig until it comes out. Unbelievable. Should dig till it comes out})} & \pbox{0.15\textwidth}{{[}"đéo", "cào", "cào"]\\(\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{Eng}}}}}}}}}}}}}}}}: ["\textit{fucking}", "\textit{dig}", "\textit{dig}"])}                                 & \pbox{0.15\textwidth}{{[}"đéo"]\\(\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{Eng}}}}}}}}}}}}}}}}: ["\textit{fucking}"])}                                                                  & \pbox{0.15\textwidth}{{[}"đéo"]\\(\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{Eng}}}}}}}}}}}}}}}}}}}}}}}}}}}}}}}}: ["\textit{fucking}"])}     \\
\hline
\end{tabular}
}
\end{table*}
